Simulating Tracking Data to Advance Sports Analytics Research

Advanced analytics have transformed how sports teams operate, particularly in episodic sports like baseball. Their impact on continuous invasion sports, such as soccer and ice hockey, has been limited due to increased game complexity and restricted access to high-resolution game tracking data. In this demo, we present a method to collect and utilize simulated soccer tracking data from the Google Research Football environment to support the development of models designed for continuous tracking data. The data is stored in a schema that is representative of real tracking data and we provide processes that extract high-level features and events. We include examples of established tracking data models to showcase the efficacy of the simulated data. We address the scarcity of publicly available tracking data, providing support for research at the intersection of artificial intelligence and sports analytics.

==> data_features.tex <==
\section{Dataset Features}
\label{sec:data_features}

\begin{itemize}
    \item Show data distributions and plots here
\end{itemize}

==> demo_requirements.tex <==
\clearpage

\section*{Demo Setting Requirements}

Our demo will be shown on one of the author's laptops. The following resources are required for the demo setting at the conference:

\begin{itemize}
    \item Large display with which to show our demo. For example, a monitor or television.
    \item Standard means of connecting laptop to the display. For example, an HDMI cable.
    \item Access to a power source.
\end{itemize}

\newpage

==> related_work.tex <==
\section{Related Work}
\label{sec:related_work}

\begin{itemize}
    \item Talk about existing tracking systems, hard to get actual data as researchers

    \item Discuss existing work using tracking data: tracking xG, EPV, pitch control, beyond xG...

    \item Big data bowl, big data cup, events with public tracking data but not regularly made public and just samples.
\end{itemize}

Despite limited access to public tracking data, invasion game sports like football, 

==> reviews.tex <==
Review 1

he paper introduces a Python based toolkit that enable the extraction of tracking- (e.g. information about player and ball position, speed and direction of movement) and event- (e.g. passes, shots, goals, interceptions) data from the Google Research Footbal (GRF) Reinforcement Learning simulated environment.

The main motivation for the development of this toolkit is the lack of access to tracking data from real world games, which hinders the potential for more research in communities interested in team sports analytics. The collected data is stored in a schema claimed to be representative of real world tracking data.

The demo video showcases how the collected data can be leveraged to create prediction models that are commonly used in sports analytics, such as Expected Goals (xG - the probability of making a goal when shooting the ball from a given distance and angle) or Pitch Control (the probability that a team will hold possession of the ball given the spatial pitch region in which the ball is placed and the concentration of team players around it).

The paper is relevant for research communities at the intersection of agent-based simulation and sports analytics.

Nonetheless, the contribution would have been stronger if some details about the data collection schema were given or the degree of it "immitating" real world tracking data. Is the schema employed for GRF specific to that environment or is it more general? The contribtion could also better highlight if the prediction models that are provided within the toolkit carry any real prediction accuracy (e.g. with respect to an set of simulated game playouts for player agents following a given strategy).

Rating: 7: Good paper, accept

Confidence: 4: The reviewer is confident but not absolutely certain that the evaluation is correct

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Review 2

The work discussed in this paper seems to fill an important gap in public research into invasion games like hockey and football. As such, the work is an important contribution and worthy of presenting. The resulting visuals that are produced are also informative and intuitive to understand and therefore very helpful in presenting the work. However, the technique itself is unfortunately not demonstrable or interactive, if I understand it well. The software that generates the simulation data and extracts expected goals or pitch control features simply runs in a command line tool, where not much is to be seen. The code can be shown of course, but that is not a demonstration. What is shown is the results of the technique, some of which could be shown in a paper, although the animated passes for example could not. Hence I still believe it would be an interesting demo to show at AAMAS.

Rating: 7: Good paper, accept

Confidence: 4: The reviewer is confident but not absolutely certain that the evaluation is correct
